Search for effective Lorentz and CPT violation using ZEUS data

Lorentz and CPT symmetry in the quark sector of the Standard Model are studied in the context of an effective field theory using ZEUS $e^{\pm} p$ data. Symmetry-violating effects can lead to time-dependent oscillations of otherwise time-independent observables, including scattering cross sections. An analysis using five years of inclusive neutral-current deep inelastic scattering events corresponding to an integrated HERA luminosity of $372\; \text{pb}^{-1}$ at $\sqrt{s} = 318$ Gev has been performed. No evidence for oscillations in sidereal time has been observed within statistical and systematic uncertainties. Constraints, most for the first time, are placed on 42 coefficients parameterising dominant CPT-even dimension-four and CPT-odd dimension-five spin-independent modifications to the propagation and interaction of light quarks.

==> LaTeX/zeus/zeus_def.tex <==
%------------------------------------------------------------------------------
%       Standard ZEUS text fragments
%       ----------------------------
%       -> references system footnote
%------------------------------------------------------------------------------
\newcommand{\ZcoosysA}{%
The ZEUS coordinate system is a right-handed Cartesian system, with the $Z$
axis pointing in the proton beam direction, referred to as the ``forward
direction'', and the $X$ axis pointing left towards the center of HERA.
The coordinate origin is at the nominal interaction point.\xspace}
\newcommand{\ZcoosysB}{%
The ZEUS coordinate system is a right-handed Cartesian system, with the $Z$
axis pointing in the proton beam direction, referred to as the ``forward
direction'', and the $X$ axis pointing left towards the centre of HERA.
The coordinate origin is at the nominal interaction point.\xspace}
\newcommand{\Zpsrap}{%
The pseudorapidity is defined as $\eta=-\ln\left(\tan\frac{\theta}{2}\right)$,
where the polar angle, $\theta$, is measured with respect to the proton beam
direction.\xspace}
\newcommand{\ZcoosysfnA}{\footnote{\ZcoosysA}}
\newcommand{\ZcoosysfnB}{\footnote{\ZcoosysB}}
\newcommand{\ZcoosysfnAeta}{\footnote{\ZcoosysA\Zpsrap}}
\newcommand{\ZcoosysfnBeta}{\footnote{\ZcoosysB\Zpsrap}}
%------------------------------------------------------------------------------
%       -> introductory sentence for detector description
%------------------------------------------------------------------------------
\newcommand{\Zdetdesc}{%
A detailed description of the ZEUS detector can be found 
elsewhere~\cite{zeus:1993:bluebook}. A brief outline of the 
components that are most relevant for this analysis is given
below.\xspace}
%------------------------------------------------------------------------------
%       -> CTD description (coordinate system footnote is given as argument)
%------------------------------------------------------------------------------
\newcommand{\Zctddesc}[1]{%
Charged particles were tracked in the central tracking detector (CTD)~\citeCTD,
which operated in a magnetic field of $1.43\Tesla$ provided by a thin 
superconducting coil. The CTD consisted of 72~cylindrical drift chamber 
layers, organized in 9~superlayers covering the polar-angle#1 region 
\mbox{$15^\circ<\theta<164^\circ$}. The transverse-momentum resolution for
full-length tracks is $\sigma(p_T)/p_T=0.0058p_T\oplus0.0065\oplus0.0014/p_T$,
with $p_T$ in $\Gev$.}
%------------------------------------------------------------------------------
%       -> CTD/MVD description (coordinate system footnote is given as argument)
%------------------------------------------------------------------------------
\newcommand{\Zctdmvddesc}[1]{%
In the kinematic range of the analysis, charged particles were tracked
in the central tracking detector (CTD)~\citeCTD, and the microvertex
detector (MVD)~\citeMVD. These components operated in a magnetic
field of $1.43\Tesla$ provided by a thin superconducting solenoid. The
CTD consisted of 72~cylindrical drift chamber layers, organised in
nine superlayers covering the polar-angle#1 region
\mbox{$15^\circ<\theta<164^\circ$}. The MVD consisted of a barrel
(BMVD) and a forward (FMVD) section with three cylindrical layers and
four vertical planes of single-sided silicon strip sensors in the BMVD
and FMVD respectively. The BMVD provided polar-angle coverage for
tracks with three measurements from $30^\circ$ to $150^\circ$. The
FMVD extended the polar-angle coverage in the forward region to
$7^\circ$. After alignment the single hit resolution of the BMVD was
$\rm 25\,\mu m$ and the impact parameter resolution of the CTD-BMVD system
for high momentum tracks was $\rm 100\,\mu m$.}
%------------------------------------------------------------------------------
%       -> CTD/MVD/STT description (coordinate system footnote is given as argument)
%------------------------------------------------------------------------------
\newcommand{\Zctdmvdsttdesc}[1]{%
In the kinematic range of the analysis, charged particles were tracked
in the central tracking detector (CTD)~\citeCTD, the microvertex
detector (MVD)~\citeMVD and the STT~\citeSTT. The CTD and the MVD
operated in a magnetic field of $1.43\Tesla$ provided by a thin
superconducting solenoid. The CTD drift chamber covered the
polar-angle#1 region \mbox{$15^\circ<\theta<164^\circ$}. The MVD
silicon tracker consisted of a barrel (BMVD) and a forward (FMVD)
section. The BMVD provided polar angle coverage for tracks with three
measurements from $30^\circ$ to $150^\circ$. The FMVD extended the
polar-angle coverage in the forward region to $7^\circ$. The STT
covered the polar-angle region \mbox{$5^\circ<\theta<25^\circ$}.}
%------------------------------------------------------------------------------
%       -> CTD/MVD/STT description (coordinate system footnote is given as argument)
%------------------------------------------------------------------------------
\newcommand{\Zsttdesc}[1]{%
The STT consisted of 48 sectors of two different sizes. Each sector
contained 192 (small sector) or 264 (large sector) straws of diameter
7.5 mm arranged into 3 layers. The sectors were trapezoidal in shape
and each subtended an azimuthal angle of $60^{\circ}$ -- 6 sectors
formed a so-called superlayer. A particle passing through the complete
detector traversed 8 superlayers, which were rotated around the beam
direction at angles of $30^{\circ}$ or $15^{\circ}$ to each other. The STT
covered the polar-angle region $5^{\circ}<\theta<23^{\circ}$.
}
%------------------------------------------------------------------------------
%       -> CAL description
%------------------------------------------------------------------------------
\newcommand{\Zcaldesc}{%
The high-resolution uranium--scintillator calorimeter (CAL)~\citeCAL consisted 
of three parts: the forward (FCAL), the barrel (BCAL) and the rear (RCAL)
calorimeters. Each part was subdivided transversely into towers and
longitudinally into one electromagnetic section (EMC) and either one (in RCAL)
or two (in BCAL and FCAL) hadronic sections (HAC). The smallest subdivision of
the calorimeter is called a cell.  The CAL energy resolutions, as measured under
test-beam conditions, are $\sigma(E)/E=0.18/\sqrt{E}$ for electrons and
$\sigma(E)/E=0.35/\sqrt{E}$ for hadrons ($E$ in $\Gev$).}
%------------------------------------------------------------------------------
%       -> HES description
%------------------------------------------------------------------------------
\newcommand{\Zhesdesc}{%
The position of electrons scattered at small angles to the
electron-beam directions was determined with the help of RHES\citeHES,
which consisted of a layer of approximately $10\,000$ $(2.96\times
3.32\,{\rm cm^2})$ silicon-pad detectors inserted in the RCAL at a
depth of 3.3 radiation lengths.}
%------------------------------------------------------------------------------
%       -> MUON description
%------------------------------------------------------------------------------
\newcommand{\Zmuondesc}{%
The muon system consisted of rear, barrel (R/BMUON) and forward
(FMUON) tracking detectors. The B/RMUON consisted of limited--streamer
(LS) tube chambers placed behind the BCAL (RCAL), inside and outside a
magnetized iron yoke surrounding the CAL. The barrel and rear muon
chambers cover polar angles from $34^\circ$ to $135^\circ$ and from
$135^\circ$ to $171^\circ$, respectively. The FMUON consisted of six
trigger planes of LS tubes and four planes of drift chambers covering
the angular region from $5^\circ$ to $32^\circ$. The muon system
exploited the magnetic field of the iron yoke and, in the forward
direction, of two iron toroids magnetized to $\approx\,1.6\,{\rm T}$
to provide an independent measurement of the muon momentum.}
%------------------------------------------------------------------------------
%       -> BAC description
%------------------------------------------------------------------------------
\newcommand{\Zbacdesc}{%
The iron yoke surrounding the CAL was instrumented with proportional
drift chambers to form the Backing Calorimeter (BAC)~\citeBAC.  The
BAC consisted of 5142 aluminium chambers inserted into the gaps
between $7.3\,{\rm cm}$ thick iron plates (10, 9 and 7 layers in forecap,
barrel and rearcap, respectively) serving as calorimeter absorber.
The chambers were typically $5\,{\rm m}$ long and had a wire spacing of
$1.5\,{\rm cm}$. The anode wires were covered by $50\,{\rm cm}$ long cathode
pads. The BAC was equipped with energy
readout and position sensitive readout for muon tracking.  The former
was based on 1692 pad towers ($50 \times 50\,{\rm cm^2}$), providing an
energy resolution of $\sim 100\%/\sqrt E$. The position information
from the wires allowed the reconstruction of muon trajectories in two
dimensions ($XY$ in barrel and $YZ$ in endcaps) with spatial accuracy
of a few mm.}
%------------------------------------------------------------------------------
%       -> LUMI description (The actual lumi uncertainty in percent is given as the argument) 
%------------------------------------------------------------------------------
\newcommand{\Zlumidesc}[1]{%
The luminosity was measured using the Bethe-Heitler reaction
$ep\,\rightarrow\, e\gamma p$ by a luminosity detector which consisted
of independent lead-scintillator calorimeter\citePCAL and a magnetic
spectrometer\citeSPECTRO systems. The fractional systematic
uncertainty on the measured luminosity was #1.}
%------------------------------------------------------------------------------
%       -> 6mT description
%------------------------------------------------------------------------------
%\newcommand{\Z6mTdesc}{%
%Scattered electrons emerging from $eP$ interactions at very small
%angles were detected in a small tungsten--scintillator calorimeter
%located approximately 6~m from the interaction point in the rear
%direction, referred to as the ``6m-tagger''~\cite6mT. For
%electrons in the energy range $4.1\le E_e\le7.4$ the acceptance is 
%very close to one with very high purity.}
%------------------------------------------------------------------------------
%       -> Standard Acknowledgements
%------------------------------------------------------------------------------
\newcommand{\Zacknowledge}{%
We appreciate the contributions to the construction and maintenance of the 
ZEUS de- tector of many people who are not listed as authors. The HERA 
machine group and the DESY computing staff are especially acknowledged for 
their success in providing excel- lent operation of the collider and the 
data-analysis environment. We thank the DESY directorate for their strong 
support and encouragement.}
%------------------------------------------------------------------------------
%       Handy macros, mainly for text mode:
%       -----------------------------------
%       -> unknown marker
%------------------------------------------------------------------------------
\newcommand{\xxx}{\hbox{$\qsm\qsm\qsm$}\xspace}
%------------------------------------------------------------------------------
%       -> D0 acronym
%------------------------------------------------------------------------------
\newcommand{\DO}{{D{\O}}\xspace}
%------------------------------------------------------------------------------
%       -> (anti-)something with correct hyphenation
%------------------------------------------------------------------------------
\newcommand{\Anti}[1]{\hbox{(anti-)}\discretionary{}{}{}#1}
\newcommand{\anti}[1]{(anti\discretionary{-)}{}{)}#1}
%------------------------------------------------------------------------------
%       -> characters for typewriter font (used for http addresses)
%------------------------------------------------------------------------------
\chardef\usc=95
\chardef\til=126
%------------------------------------------------------------------------------
%       -> xdotspace (like xspace, but adds period unless
%          another period follows)
%       -> "nn% C.L."
%------------------------------------------------------------------------------
\catcode`\@=11 % @ signs are now treated as letters
\DeclareRobustCommand\xdotspace{\futurelet\@let@token\@xdotspace}
\def\@xdotspace{%
  \ifx\@let@token.\else
  \ifx\@let@token\bgroup.\else
  \ifx\@let@token\egroup.\else
  \ifx\@let@token\/.\else
  \ifx\@let@token\ .\else
  \ifx\@let@token~.\else
  \ifx\@let@token!.\else
  \ifx\@let@token,.\else
  \ifx\@let@token:.\else
  \ifx\@let@token;.\else
  \ifx\@let@token?.\else
  \ifx\@let@token/.\else
  \ifx\@let@token'.\else
  \ifx\@let@token).\else
  \ifx\@let@token-.\else
  \ifx\@let@token\@xobeysp.\else
  \ifx\@let@token\space.\else
  \ifx\@let@token\@sptoken.\else
   .\space
   \fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi}
\catcode`\@=12 % @ signs are no longer letters
\newcommand{\CL}[1]{$#1\%$~C.L\xdotspace}
%------------------------------------------------------------------------------
%       -> vertical rule of width zero and variable height & depth
%------------------------------------------------------------------------------
\newcommand{\stru}[2]{%
   \relax\ifmmode\hbox{\vrule height#1 depth#2 width0pt}%
   \else\vrule height#1 depth#2 width0pt\fi}
%------------------------------------------------------------------------------
%       -> underline with resonable distance text - line
%------------------------------------------------------------------------------
\newcommand{\uline}[1]{$\underline{\hbox{#1\stru{0.pt}{.485ex}}}$}
%------------------------------------------------------------------------------
%       -> roman numbers (uppercase and lowercase)
%------------------------------------------------------------------------------
\newcommand{\Ronum}[1]{\uppercase\expandafter{\romannumeral#1}}
\newcommand{\ronum}[1]{\expandafter{\romannumeral#1}}
%------------------------------------------------------------------------------
%       -> definition for LaTeX4zeus
%------------------------------------------------------------------------------
\DeclareRobustCommand{\LaTeXZ}{%
  \LaTeX\kern-.05em4\kern-.1em
  {\raisebox{-0.2ex}{$\scriptstyle\text{ZEUS}$}}\xspace}
%------------------------------------------------------------------------------
%       -> umlaut definitions for references (needed since BiBTeX 
%          MACRO strings cannot contain quotes)
%------------------------------------------------------------------------------
\newcommand{\Auml}{\"A}
\newcommand{\Ouml}{\"O}
\newcommand{\Uuml}{\"U}
\newcommand{\auml}{\"a}
\newcommand{\ouml}{\"o}
\newcommand{\uuml}{\"u}
%------------------------------------------------------------------------------
%       -> shorthands for equation, figure, table, section references
%          (require standard use of labels: eq-... for equations, cha-...
%           for chapters, sec-... for (sub)sections, tab-... for tables
%           and fig-... for figures)
%------------------------------------------------------------------------------
\newcommand{\eq}[1]{(\ref{eq-#1})}
\newcommand{\eqsand}[2]{(\ref{eq-#1}) and~(\ref{eq-#2})}
\newcommand{\eqsto}[2]{(\ref{eq-#1})--(\ref{eq-#2})}
\newcommand{\eqstwo}[2]{(\ref{eq-#1},\ref{eq-#2})}
\newcommand{\eqsthr}[3]{(\ref{eq-#1},\ref{eq-#2},\ref{eq-#3})}
\newcommand{\eqsfou}[4]{(\ref{eq-#1},\ref{eq-#2},\ref{eq-#3},\ref{eq-#4})}
\newcommand{\Eq}[1]{Equation~(\ref{eq-#1})}
\newcommand{\Eqsto}[2]{Equations~(\ref{eq-#1})--(\ref{eq-#2})}
\newcommand{\fig}[1]{Fig.~\ref{fig-#1}}
\newcommand{\Fig}[1]{Figure~\ref{fig-#1}}
\newcommand{\figand}[2]{Figs.~\ref{fig-#1} and~\ref{fig-#2}}
\newcommand{\Figand}[2]{Figures~\ref{fig-#1} and~\ref{fig-#2}}
\newcommand{\tab}[1]{Table~\ref{tab-#1}}
\newcommand{\Tab}[1]{Table~\ref{tab-#1}}
\newcommand{\taband}[2]{Tables~\ref{tab-#1} and~\ref{tab-#2}}
\newcommand{\cha}[1]{Chap.~\ref{cha-#1}}
\newcommand{\Cha}[1]{Chapter~\ref{cha-#1}}
\newcommand{\sect}[1]{Sect.~\ref{sec-#1}}
\newcommand{\Sect}[1]{Section~\ref{sec-#1}}
\newcommand{\sectand}[2]{Sects.~\ref{sec-#1} and~\ref{sec-#2}}
\newcommand{\sectto}[2]{Sects.~\ref{sec-#1} to~\ref{sec-#2}}
\newcommand{\Sectand}[2]{Sections~\ref{sec-#1} and~\ref{sec-#2}}
\newcommand{\Sectto}[2]{Sections~\ref{sec-#1} to~\ref{sec-#2}}
%------------------------------------------------------------------------------
%       -> log file message
%------------------------------------------------------------------------------
\newcommand{\LogMess}[1]{\typeout{^^J==> #1^^J}}
%------------------------------------------------------------------------------
%       Some special symbols and settings for math mode:
%       ------------------------------------------------
%       -> redefine mathbf
%------------------------------------------------------------------------------
\DeclareMathAlphabet{\mathbf}{OT1}{cmr}{bx}{sl}
%------------------------------------------------------------------------------
%       -> physics units (eV and multiples)
%------------------------------------------------------------------------------
\newcommand{\eVdist}{\kern-0.06667em}
\newcommand{\Ev}{{\text{e}\eVdist\text{V\/}}}
\newcommand{\Kev}{{\text{ke}\eVdist\text{V\/}}}
\newcommand{\Mev}{{\text{Me}\eVdist\text{V\/}}}
\newcommand{\Gev}{{\text{Ge}\eVdist\text{V\/}}}
\newcommand{\Tev}{{\text{Te}\eVdist\text{V\/}}}
\newcommand{\ev}{{\,\text{e}\eVdist\text{V\/}}}
\newcommand{\kev}{{\,\text{ke}\eVdist\text{V\/}}}
\newcommand{\mev}{{\,\text{Me}\eVdist\text{V\/}}}
\newcommand{\gev}{{\,\text{Ge}\eVdist\text{V\/}}}
\newcommand{\tev}{{\,\text{Te}\eVdist\text{V\/}}}
%------------------------------------------------------------------------------
%       -> various other units
%------------------------------------------------------------------------------
\newcommand{\mb}{\,\text{mb}}
\newcommand{\mub}{\,\upmu\text{b}}
\newcommand{\nb}{\,\text{nb}}
\newcommand{\pb}{\,\text{pb}}
\newcommand{\fb}{\,\text{fb}}
\newcommand{\mubi}{\,\upmu\text{b}^{-1}}
\newcommand{\mbi}{\,\text{mb}^{-1}}
\newcommand{\nbi}{\,\text{nb}^{-1}}
\newcommand{\pbi}{\,\text{pb}^{-1}}
\newcommand{\fbi}{\,\text{fb}^{-1}}
\newcommand{\met}{\,\text{m}}
% \newcommand{\nm}{\,\text{nm}}
\newcommand{\mum}{\,\upmu\text{m}}
% \newcommand{\mm}{\,\text{mm}}
% \newcommand{\cm}{\,\text{cm}}
\newcommand{\km}{\,\text{km}}
\newcommand{\Amp}{\,\text{A}}
\newcommand{\nA}{\,\text{nA}}
\newcommand{\muA}{\,\upmu\text{A}}
\newcommand{\mA}{\,\text{mA}}
\newcommand{\kA}{\,\text{kA}}
% \newcommand{\Hz}{\,\text{Hz}}
% \newcommand{\kHz}{\,\text{kHz}}
% \newcommand{\MHz}{\,\text{MHz}}
% \newcommand{\GHz}{\,\text{GHz}}
\newcommand{\ppm}{\,\text{ppm}}
\newcommand{\ppb}{\,\text{ppb}}
\newcommand{\scd}{\,\text{s}}
% \newcommand{\ps}{\,\text{ps}}
% \newcommand{\ns}{\,\text{ns}}
\newcommand{\mus}{\,\upmu\text{s}}
\newcommand{\ms}{\,\text{ms}}
% \newcommand{\rad}{\,\text{rad}}
\newcommand{\murad}{\,\upmu\text{rad}}
% \newcommand{\mrad}{\,\text{mrad}}
\newcommand{\gra}{\,\text{g}}
\newcommand{\pg}{\,\text{pg}}
\newcommand{\nang}{\,\text{ng}}
\newcommand{\mug}{\,\upmu\text{g}}
\newcommand{\mg}{\,\text{mg}}
\newcommand{\kg}{\,\text{kg}}
\newcommand{\Tesla}{\,\text{T}}
\newcommand{\Kelvin}{\,\text{K}}
%------------------------------------------------------------------------------
%       -> additional operators
%------------------------------------------------------------------------------
\newcommand{\odiv}{{\operatorname*{div}}}
\newcommand{\ograd}{{\operatorname*{grad}}}
\newcommand{\orot}{{\operatorname*{rot}}}
\newcommand{\odiag}{{\operatorname*{diag}}}
\newcommand{\ocov}{{\operatorname*{cov}}}
%------------------------------------------------------------------------------
%       -> fraction with slash instead of ratio bar
%------------------------------------------------------------------------------
\newcommand{\slashfrac}[2]{%
  \raisebox{0.5ex}{\ensuremath #1}\kern-0.12em/\kern-0.08em
  \raisebox{-.8ex}{\ensuremath #2}}
%------------------------------------------------------------------------------
%       -> shorthand for "integral limits below and above"
%------------------------------------------------------------------------------
\newcommand{\intl}{\int\limits}
\newcommand{\ointl}{\oint\limits}
%------------------------------------------------------------------------------
%       -> d'Alembert operator
%------------------------------------------------------------------------------
\newcommand{\sqr}[3]{%
    {\vcenter{\hrule height.#3ex\hbox{\vrule width.#2ex height#1ex
     \kern#1ex\vrule width.#3ex}\hrule height.#2ex}}}
\newcommand{\dalem}{\mathchoice\sqr{1.3}{08}{24}\sqr{1.4}{08}{24}
                    \sqr{1.15}{07}{21}\sqr{1.0}{06}{18}\,}
%------------------------------------------------------------------------------
%       -> vectors and matrices
%------------------------------------------------------------------------------
\newcommand{\vect}[1]{\begin{matrix}#1\end{matrix}}
\newcommand{\pvect}[1]{\begin{pmatrix}#1\end{pmatrix}}
\newcommand{\bvect}[1]{\begin{bmatrix}#1\end{bmatrix}}
\newcommand{\vvect}[1]{\begin{vmatrix}#1\end{vmatrix}}
\newcommand{\Vvect}[1]{\begin{Vmatrix}#1\end{Vmatrix}}
%------------------------------------------------------------------------------
%       -> antiparticles and particles with a bar in parentheses
%------------------------------------------------------------------------------
\newcommand{\widebar}[1]{%
   \mkern1.5mu\overline{\mkern-1.5mu#1\mkern-1.mu}\mkern1.mu}
\catcode`\@=11 % @ signs are now treated as letters
\newcommand{\parenbar}{\mathpalette\p@renb@r}
\def\p@renb@r#1#2{\vbox{%
  \ifx#1\scriptscriptstyle \dimen@.7em\dimen@ii.2em\else
  \ifx#1\scriptstyle \dimen@.8em\dimen@ii.25em\else
  \dimen@1em\dimen@ii.4em\fi\fi \offinterlineskip
  \ialign{\hfill##\hfill\cr
    \vbox{\hrule width\dimen@ii}\cr
    \noalign{\vskip-.3ex}%
    \hbox to\dimen@{$\mathchar300\hfil\mathchar301$}\cr
    \noalign{\vskip-.3ex}%
    $#1#2$\cr}}}
\catcode`\@=12 % @ signs are no longer letters
\newcommand{\nuan}{\parenbar{\nu}}
\newcommand{\nunubar}{\parenbar{\nu}}
\newcommand{\ppbar}{\parenbar{p}}
\newcommand{\qqbar}{\parenbar{q}}
\newcommand{\pbar}{\widebar{p}}
\newcommand{\nbar}{\widebar{n}}
\newcommand{\qbar}{\widebar{q}}
\newcommand{\dbar}{\widebar{d}}
\newcommand{\ubar}{\widebar{u}}
\newcommand{\sbar}{\widebar{s}}
\newcommand{\cbar}{\widebar{c}}
% \newcommand{\bbar}{\widebar{b}}
\newcommand{\tbar}{\widebar{t}}
\newcommand{\nubar}{\widebar{\nu}}
\newcommand{\Dbar}{\widebar{D}}
\newcommand{\ebar}{\widebar{e}}
\newcommand{\Ebar}{\widebar{e}}
\newcommand{\Hebar}{\widebar{\text{He}}}
\newcommand{\Cbar}{\widebar{\text{C}}}
\newcommand{\Abar}{\widebar{\text{A}}}
\newcommand{\Kbar}{\widebar{K}}
\newcommand{\chibar}{\widebar{\chi}}
\newcommand{\LQbar}{\widebar{\rm LQ}}
%------------------------------------------------------------------------------
%       -> small numbers
%------------------------------------------------------------------------------
\newcommand{\zero}{{\scriptscriptstyle 0}}
\newcommand{\sone}{{\scriptscriptstyle 1}}
\newcommand{\stwo}{{\scriptscriptstyle 2}}
\newcommand{\sthr}{{\scriptscriptstyle 3}}
\newcommand{\sfou}{{\scriptscriptstyle 4}}
\newcommand{\sfiv}{{\scriptscriptstyle 5}}
\newcommand{\ssix}{{\scriptscriptstyle 6}}
\newcommand{\ssev}{{\scriptscriptstyle 7}}
\newcommand{\seig}{{\scriptscriptstyle 8}}
\newcommand{\snin}{{\scriptscriptstyle 9}}
\newcommand{\sten}{{\scriptscriptstyle 10}}
\newcommand{\half}{{\scriptscriptstyle 1/2}}
%------------------------------------------------------------------------------
%       -> abbreviations for common math mode symbols
%------------------------------------------------------------------------------
\newcommand{\MSbar}{\hbox{$\overline{\rm MS}$}\xspace}
\newcommand{\UO}{{\rm U}(1)_\sY}
\newcommand{\SUT}{{\rm SU}(2)_\sL}
\newcommand{\SUTH}{{\rm SU}(3)_c}
\newcommand{\SUTUO}{{\rm SU}(2)_\sL\times{\rm U}(1)_\sY}
\newcommand{\SUTSUTUO}{{\rm SU}(3)_c\times{\rm SU}(2)_\sL\times{\rm U}(1)_\sY}
\newcommand{\alsmu}[1]{{\alpha_s(\mu_{#1}^2)}}
\newcommand{\alsmz}{{\alpha_s(M_Z^2)}}
\newcommand{\alsqs}{{\alpha_s(Q^2)}}
\newcommand{\als}{\alpha_s}
\newcommand{\ctwb}{\cos\theta_W}
\newcommand{\ctws}{\cos^2\theta_W}
\newcommand{\diff}{{\rm d}}
\newcommand{\gh}{{\gamma_h}}
\newcommand{\lsq}[1]{{\lambda_{#1}}}
\newcommand{\lsqp}[1]{{\lambda'_{#1}}}
\newcommand{\lsqpp}[1]{{{\lambda''}_{#1}}}
\newcommand{\rnge}{\hbox{$\,\text{--}\,$}}
\newcommand{\sihat}{{\hat\sigma}}
\newcommand{\sitil}{{\tilde\sigma}}
\newcommand{\stwb}{\sin\theta_W}
\newcommand{\stwss}{\sin^4\theta_W}
\newcommand{\stws}{\sin^2\theta_W}
\newcommand{\ta}{{\theta^\ast}}
\newcommand{\tilR}{\tilde R}
\newcommand{\tilS}{\tilde S}
\newcommand{\tilU}{\tilde U}
\newcommand{\tilV}{\tilde V}
\newcommand{\tl}{{\theta_\ell}}
\newcommand{\tw}{\theta_W}
%------------------------------------------------------------------------------
%       -> roman character combinations to be used in math mode, mainly
%          sub- or superscripts
%------------------------------------------------------------------------------
\newcommand{\Born}{{\rm Born}}
\newcommand{\BR}{{\rm BR}}
\newcommand{\CC}{{\rm CC}}
\newcommand{\CI}{{\rm CI}}
\newcommand{\CJ}{{\rm CJ}}
\newcommand{\DA}{{\rm DA}}
\newcommand{\DCA}{{\rm DCA}}
\newcommand{\GRV}{{\rm GRV}}
\newcommand{\IC}{{\rm IC}}
\newcommand{\ISR}{{\rm ISR}}
\newcommand{\IP}{{\rm I$\kern-0.01667em$P}\xspace}
\newcommand{\JB}{{\rm JB}}
\newcommand{\LL}{{\rm LL}}
\newcommand{\LQ}{{\rm LQ}}
\newcommand{\LR}{{\rm LR}}
\newcommand{\MC}{{\rm MC}}
\newcommand{\NC}{{\rm NC}}
\newcommand{\NS}{{\rm NS}}
\newcommand{\QPM}{{\rm QPM}}
\newcommand{\RL}{{\rm RL}}
\newcommand{\RPv}{{{\not R}_P}}
\newcommand{\RR}{{\rm RR}}
\newcommand{\SM}{{\rm SM}}
\newcommand{\bkg}{{\rm bkg}}
\newcommand{\cut}{{\rm cut}}
\newcommand{\data}{{\rm data}}
\newcommand{\sdet}{{\rm det}}
\newcommand{\dof}{{\rm dof}}
\newcommand{\eff}{{\rm eff}}
\newcommand{\elm}{{\rm elm}}
\newcommand{\evt}{{\rm evt}}
\newcommand{\exc}{{\rm exc}}
\newcommand{\fit}{{\rm fit}}
\newcommand{\had}{{\rm had}}
\newcommand{\jet}{{\rm jet}}
\newcommand{\meas}{{\rm meas}}
\newcommand{\miss}{{\rm miss}}
\newcommand{\obs}{{\rm obs}}
\newcommand{\pnt}{{\rm pnt}}
\newcommand{\sL}{{\rm L}}
\newcommand{\sR}{{\rm R}}
\newcommand{\sS}{{\rm S}}
\newcommand{\sT}{{\rm T}}
\newcommand{\sY}{{\rm Y}}
\newcommand{\sca}{{\rm sca}}
\newcommand{\sexp}{{\rm exp}}
\newcommand{\sint}{{\rm int}}
\newcommand{\smin}{{\rm min}}
\newcommand{\smax}{{\rm max}}
\newcommand{\srad}{{\rm rad}}
\newcommand{\sthe}{{\rm the}}
\newcommand{\sys}{{\rm sys}}
\newcommand{\tot}{{\rm tot}}
\newcommand{\true}{{\rm true}}
%------------------------------------------------------------------------------
%       -> some calligraphic symbols and applications
%------------------------------------------------------------------------------
\newcommand{\Cor}{{\cal C}}
\newcommand{\F}{{\cal F}}
\newcommand{\Lumi}{{\cal L}}
\newcommand{\Prob}{{\cal P}}
\newcommand{\ord}[1]{{\cal O}(#1)}
\newcommand{\ordlr}[1]{{\cal O}\left(#1\right)}
%------------------------------------------------------------------------------
%       -> some math symbols (+,-,...) for usage as mathchar's
%------------------------------------------------------------------------------
\mathchardef\qsm=63
\mathchardef\pls=43
\mathchardef\mns=512
\mathchardef\plm=518
\mathchardef\eql=61
\mathchardef\smallleft=300
\mathchardef\smallright=301
\mathchardef\les=316
\mathchardef\gre=318
\mathchardef\leq=532
\mathchardef\grq=533
%------------------------------------------------------------------------------
%       Additional functionality for tables and figures
%       -----------------------------------------------
%       -> alignment tools for tables
%------------------------------------------------------------------------------
\newcommand{\cA}{{\phantom{0}}}
\newcommand{\cB}{{\phantom{00}}}
\newcommand{\cC}{{\phantom{000}}}
\newcommand{\cD}{{\phantom{0000}}}
\newcommand{\cAp}{{\phantom{0.}}}
\newcommand{\cM}{{\phantom{\mns}}}
\newcommand{\cP}{{\phantom{\pls}}}
%------------------------------------------------------------------------------
%       -> comments on figures (allow to add axodraw and picture items)
%------------------------------------------------------------------------------
\catcode`\@=11 % @ signs are now treated as letters
\newcounter{pict@width}
\newcounter{pict@height}
\newlength{\pict@scale}
\setlength{\pict@scale}{0.1mm}
\newcommand{\psfigadd}[4]{%
\setcounter{pict@width}{1*\ratio{#2+\pict@scale/2}{\pict@scale}}
\setcounter{pict@height}{1*\ratio{#3+\pict@scale/2}{\pict@scale}}
\setlength{\unitlength}{\pict@scale}
\hbox to #2{\hspace{-\fill}\begin{picture}(\thepict@width,\thepict@height)
\put(0,0){\psfig{figure=#1,width=#2,height=#3,clip=}}
\SetScale{0.283466457}
\SetWidth{1.763889}
{#4}
\end{picture}}
}
\newcounter{pict@widthfst}
\newcounter{pict@widthscd}
\newcounter{pict@widthtot}
\newcommand{\psfigaddtwo}[7]{%
\setcounter{pict@widthfst}{1*\ratio{#2+\pict@scale/2}{\pict@scale}}
\setcounter{pict@widthscd}{1*\ratio{#2+#4+\pict@scale/2}{\pict@scale}}
\setcounter{pict@widthtot}{1*\ratio{#2+#4+#6+\pict@scale/2}{\pict@scale}}
\setcounter{pict@height}{1*\ratio{#3+\pict@scale/2}{\pict@scale}}
\setlength{\unitlength}{\pict@scale}
\hbox{\hspace{-\fill}\begin{picture}(\thepict@widthtot,\thepict@height)
\put(0,0){\psfig{figure=#1,width=#2,height=#3,clip=}}
\put(\thepict@widthscd,0){\psfig{figure=#5,width=#6,height=#3,clip=}}
\SetScale{0.283466457}
\SetWidth{1.763889}
{#7}
\end{picture}}
}
\newcommand{\psfigror}[4]{%
\setcounter{pict@width}{1*\ratio{#2+\pict@scale/2}{\pict@scale}}
\setcounter{pict@height}{1*\ratio{#3+\pict@scale/2}{\pict@scale}}
\setlength{\unitlength}{\pict@scale}
\hbox{\begin{picture}(\thepict@width,\thepict@height)
\put(0,\thepict@height){\psfig{figure=#1,width=#3,height=#2,clip=,angle=270}}
\SetScale{0.283466457}
\SetWidth{1.763889}
{#4}
\end{picture}}
}
\newcommand{\psfigrol}[4]{%
\setcounter{pict@width}{1*\ratio{#2+\pict@scale/2}{\pict@scale}}
\setcounter{pict@height}{1*\ratio{#3+\pict@scale/2}{\pict@scale}}
\setlength{\unitlength}{\pict@scale}
\hbox{\begin{picture}(\thepict@width,\thepict@height)
\put(0,0){\psfig{figure=#1,width=#3,height=#2,clip=,angle=90}}
\SetScale{0.283466457}
\SetWidth{1.763889}
{#4}
\end{picture}}
}
\catcode`\@=12 % @ signs are no longer letters
%------------------------------------------------------------------------------
%       -> narrow figures in list environment
%------------------------------------------------------------------------------
\newlength\listtextwidth
\newcommand{\shiftfloat}[1]{
  \setlength{\listtextwidth}{\textwidth}
  \addtolength{\listtextwidth}{-#1}}
%------------------------------------------------------------------------------
%       -> "none" marker
%------------------------------------------------------------------------------
\newcommand{\none}{\hbox{---}}
%------------------------------------------------------------------------------
%       -> protected commands in captions
%------------------------------------------------------------------------------
\newcommand{\pcite}[1]{{\protect\cite{#1}}}
\newcommand{\pnl}{\protect{\newline}}
%------------------------------------------------------------------------------
%       -> pseudo-footnotes for tables
%------------------------------------------------------------------------------
\catcode`\@=11 % @ signs are now treated as letters
\newlength{\@tabfninsert}
\newlength{\@tabfnwidth}
\newcommand{\tabfootnote}[2]{%
  \setlength{\@tabfninsert}{0.8em}
  \setlength{\@tabfnwidth}{\textwidth}
  \addtolength{\@tabfnwidth}{-\@tabfninsert}
  \addtolength{\@tabfnwidth}{-0.4em}
  \noindent\makebox[\@tabfninsert][r]{\footnotesize$^{#1}$\hfil}\hfill%
  \parbox[t]{\@tabfnwidth}{\footnotesize #2\hfill}}
\catcode`\@=12 % @ signs are no longer letters


==> ZEUS_LV-analysis.tex <==
\section{Experimental set-up}
\label{sec:analysis}
The analysis is based on events from the 
full high-luminosity HERA II period (2003-2007) 
with proton beam energy $E_p=920$\;GeV and 
electron/positron beam energy $E_e = 27.5$\;GeV, representing
an integrated luminosity of 372\;pb$^{-1}$. 

"The NC DIS data sample used in this analysis was taken with the ZEUS
  detector at HERA during 2003–2007 (HERA II). During this period,
  the HERA accelerator collided 27.5 GeV electron/positron  beams
  with 920 GeV proton beams, which yields a nominal centre-of- mass energy
  of s = 318 GeV. The integrated luminosity recorded by ZEUS in HERA II
  at this energy is 366 ± 7 pb −1 . A detailed description of the ZEUS
  detector can be found elsewhere~\cite{Holm:1993frx}.

\subsection{Data selection}
%
Events are chosen to satisfy the 
following criteria (electron method reconstruction)~\cite{Abramowicz:1995zi}:
\begin{itemize}
\item $Q^2 > 5 \; \GeV^2$ 
\item $E_e > 10\;\GeV$
\item $47 \; \GeV < p_z(e) < 69 \; \GeV$
\item Sinistra electron core $> 0.9$
\item scattering angle minimum $\theta(e)_{\text{min}} > 1^\circ$
\end{itemize}
This selection yields $4.5\times 10^7$ events 
covering the kinematic range 
$x\in [7.7\times 10^{-5},1]$ and $Q\in [2.2,94] \; \GeV$.
%
\subsection{Observables}
\label{ssec:observables}
%
The starting point is the triple differential DIS cross section
\footnote{Note 
the azimuthal angle of the scattered electron
$\phi$ defined in Eqs.~\eqref{xsecc},\eqref{xseca5}
is assumed to be integrated over.}

%
\begin{align}
\frac{d\sigma}{dx\; dQ \; d\phi_T},
\label{eq:startanalysis}
\end{align}
%
where the phase $\phi_T = \text{Mod}(T_\oplus,T)/T$ is 
the phase of DIS events in terms
of $T_\oplus$ and a period
of choice $T$. Within the SME, 
only $T= T_{\text{sid.}} = 23.9345$\;h 
yields a nonvanishing dependence on $\phi_T$, 
as the sidereal angle is $\omega_\oplus T_\oplus
= \tfrac{2\pi}{T_{\text{sid.}}}T_\oplus$. 
Using a different period, the time dependence 
quickly averages out; 
the larger the difference between the 
adopted test period and $T_{\text{sid.}}$, 
the faster this occurs.

It is necessary to eliminate uncertainties related to the 
instantaneous luminosity. To do so would require
the integrated luminosity to be measured roughly every minute,
however this information is not available.
Instead, the luminosity can be bypassed when 
considering double ratios of the form
%
\begin{align}
r({\mathrm  PS}_1, {\mathrm  PS}_2) = 
\frac{
\int_{{\mathrm  PS}_1 } dx dQ \frac{d\sigma}{dx\; dQ \; d\phi_T}
/
\int_{{\mathrm  PS}_1 } dx dQ d\phi_T \frac{d\sigma}{dx\; dQ \; d\phi_T}
}{
\int_{{\mathrm  PS}_2 } dx dQ \frac{d\sigma}{dx\; dQ \; d\phi_T}
/
\int_{{\mathrm  PS}_2 } dx dQ d\phi_T \frac{d\sigma}{dx\; dQ \; d\phi_T}
},
\label{r}
\end{align}
%
where ${\mathrm  PS}_1$ and ${\mathrm  PS}_2$ are 
two regions of the $(x,Q)$ phase space.
Essential properties of~\eqref{r} are 
that it is independent of the luminosity 
and equal to unity in the absence of SME effects. 
Moreover, if the regions ${\mathrm  PS}_{1,2}$ 
are chosen appropriately, the double ratio retains a 
strong $\phi_T$ dependence in the presence 
of SME effects.
As explained in Sec.~\eqref{sec:DIS}, a strong sensitivity at 
low $x$ ($\sim 10^{-5}$-$10^{-3}$) for the 
$c$-type coefficients and at moderate-to-large
$x$ ($\gtrsim 10^{-3}$)
for the $a^{(5)}$-type coefficients is expected. 
However, very low ($\lesssim 10^{-4}$) 
and semi-moderate ($\gtrsim 10^{-2}$) 
values of $x$ suffer from less DIS events
and thus larger statistical errors. 
The majority of events are sharply peaked
around $x\simeq 10^{-3}$ implying a statistically 
optimal choice of cut in $(x,Q)$ phase space.
In evaluating Eq.~\eqref{r} for 
several cut values $x_{c}$, it is found 
that the combinations simultaneously giving the 
most sensitivity to the cross section while 
producing the lowest statistics 
from the seleced data are for 
$x_c=5\times 10^{-4}$ and 
$x_{a^{(5)}}=10^{-3}$ for $c$-type 
and $a^{(5)}$-type coefficients, respectively.
However, as no higher-order QCD corrections are included 
in the cross sections~\eqref{xsecc},\eqref{xseca5},
potential large corrections are expected 
of the order $[\alpha_s (Q) \log 1/x]^n$ at very 
low $x$ that need to be resummed.  Numerically,
such effects could shift the (apparent) value of $x$ entering
the PDFs to not coincide with Bjorken $x$.
This potential issue is partially alleviated by cutting
along moderate values $x\gtrsim 10^{-3}$ where
QCD corrections have a marginal influence. The value
$x_c = 10^{-3}$ is therefore chosen for both 
the $c$- and $a^{(5)}$-type coefficients. 
In the case of the extracted 
constraints for the $c$-type coefficients 
discussed in Sec.~\ref{ssec:constraints},
negligible reduction in sensitivity compared 
to $x_c = 5\times 10^{-4}$ is observed. 

By employing Eqs.~\eqref{xsecc},\eqref{xseca5},
the phase-space integrations 
above and below $x_c = 10^{-3}$
are performed in the following manner:
\begin{align}
&\int_{{\mathrm  PS}_1 } dx dQ = 
\int_{x_c}^1 dx
\int_{Q_{\text{low}}}^{\text{min}
[Q_{\text{high}},Q_\text{max}(x)]}dQ,\\
&\int_{{\mathrm  PS}_2 } dQ dx = 
\int_{Q_{\text{low}}}^{\text{min}
[Q_{\text{max}}(x_c),Q_{\text{high}}]} dQ 
\int_{x_{\text{min}}(Q)}^{x_c} dx, 
\end{align}
where $x_{\text{min}}(Q) = Q^2/s$,
$Q_{\text{low}} = 2.2$\;GeV, $Q_{\text{high}} = 94$\;GeV,
and $Q_{\text{max}}(x) = \sqrt{xs}$. 
Performing the integrations
results in the following double ratios
%
\begin{align}
r_c(x> x_c , x< x_c ) =\; & 
1  - 11.6 \; c_u^{03}  - 13.4 \; c_u^{33} + 0.8 \;(c_u^{11} +  c_u^{22})\nonumber \\
&\phantom{1}- 3.9 \; c_d^{03}  -  2.8 \; c_d^{33} + 0.1 \; (c_d^{11} +  c_d^{22}) \; ,
\label{eq:rc}\\
r_{a^{(5)}}(x>x_c , x<x_c ) =\; & 
1 
- 6.3 \times 10^3 \; a_u^{(5)003} + 7.0 \times 10^3 \;  a_u^{(5)033}  - 2.6\times 10^3 \;  a_u^{(5)333} \nonumber   \\
& \phantom{1 } + 5.2\times 10^2 \;  (a_u^{(5)113} + a_u^{(5)223} - a_u^{(5)011}  - a_u^{(5)022}) \nonumber   \\
&
\phantom{1} - 5.1 \times 10^2 \;  a_d^{(5)003} +  5.7\times 10^2  \; a_d^{(5)033}
 - 2.1 \times 10^2  \; a_d^{(5)333}\nonumber \\
& \phantom{1 } + 47  \; (a_d^{(5)113 } + a_d^{(5)223} - a_d^{(5)011} - a_d^{(5)022} ) \; .
\label{eq:ra5}
\end{align}
%
These expressions only contain terms 
linear in the coefficients 
as higher-order corrections are greatly suppressed.
The double ratios are compared 
with analogous double ratios constructed
purely from binned DIS events. Constraints
on the coefficients may then be placed one at a time, 
setting all others to zero in accordance
with accepted procedure~\cite{tables}, after reexpressing 
the laboratory coefficients in terms of 
the SCF coefficients using Eq.~\eqref{eq:rotation}.
%
\subsection{Initial considerations}
\label{ssec:initial}
%
The main obstacle for establishing constraints on 
a potential sidereal-time dependence of the DIS 
cross section is eliminating genuine non-SME effects. 
In particular, there is a strong time dependence 
on the instantaneous luminosity, with more data taken 
between the late evening to early morning local time.
To display this effect, the 
entire DIS selection is binned using the solar phase 
$\phi_\text{solar} = 
\text{Mod}(T_\oplus,T_\text{solar})/T_\text{solar}$ 
with $T_\text{solar} =24$\;h.
In the first panel of Fig.~\ref{fig:DIS},
a plot of the resulting normalized count in 
100 $\phi_\text{solar}$ bins is shown. It is clear that 
a $\sim \pm\mathcal{O}(25\%)$ effect is present. 
Switching from solar to sidereal binning will 
dilute this solar-phase dependence 
for long data-taking periods. 
As shown in the second panel of Fig.~\ref{fig:DIS},
sidereal dilution over $\sim 5$ years 
reduces the effect by $\sim \mathcal{O}(15\%)$,
but is not sufficient to completely erase it.
The dilution effect of a much longer period of 
data taking can be simulated by binning using 
an unphysical short period. In the third 
panel of Fig.~\ref{fig:DIS}, a plot of the same 
data binned using a $T=1$\;h period is shown.
The initial solar-phase 
dependence disappears almost completely.
These effects could in principle 
be completely eliminated 
if the luminosity were measured in 
small blocks $\sim \mathcal{O}(1\;\text{min})$.
However, as mentioned in Sec.~\ref{ssec:observables}, 
this option is not available but instead can 
pursued by considering the 
luminosity-independent 
ratios~\eqref{eq:rc},\eqref{eq:ra5}
which have a strong $x$ dependence 
and represent a compromise between 
sensitivity to SME effects and the 
requirement of having a large enough number 
of events in both the numerators and denominators.

To test this strategy a ratio~\eqref{r}
is considered that does not possess 
a sizable dependence on SME effects. 
As checked by direct integration, 
the ratio $r(Q^2< Q_c^2 , Q^2 > Q^2_c )$ 
considering events with $Q^2$ 
above and below $Q_c^2 = 20$\;GeV$^2$
fulfills this requirement and 
can be used as a null test of the analysis strategy.
In each panel of Fig.~\ref{fig:DIS-20}, 
the red and blue histograms correspond to 
the normalized counts for event with $Q^2$ 
above and below 20 GeV${}^2$, respectively. 
For each choice of phase, 
these two histograms track each other and 
their ratios in the lower panels
are consistent with fluctuations around unity. 
Note that the error bars in 
the plots include only statistical uncertainties. 

An important question is whether systematic 
uncertainties are completely subdominant and can be neglected.
A partial answer can be found by performing 
Komolgorov-Smirnov (KS) tests on the binned $Q_c$ ratios. 
This test calculates the probability that the 
observed distributions are compatible with an unsorted 
sampling of a normal distribution with mean unity 
and standard deviation identical to the 
observed statistical uncertainties. Along 
with performing KS tests, 
the ratios are split into different numbers of
bins $N_{\text{bins}}$ to estimate the size of systematic 
relative to statistical effects. 
The results are presented for $T = 1$\;h in
Figs.~\ref{fig:KS-test-20-1-4} and~\ref{fig:KS-test-20-5-8};
$T = 24$\;h in Figs.~\ref{fig:KS-solar-20-1-4} and \ref{fig:KS-solar-20-5-8}; 
and $T = T_{\text{sid.}}$ in Figs.~\ref{fig:KS-sidereal-20-1-4}
and \ref{fig:KS-sidereal-20-5-8} for the data
split into 
$N_{\text{bins}} = 4, 8, 12, 16, 
25, 50, 75, \text{and}\;100$.
The error bars on the 
points only include statistical uncertainties and
the $1-\sigma$ spreads (pink bands)
are the standard deviations of the central values. 
It is observed that, independently of the 
all three cases $T = 1$\;h, $T = T_{\text{sid.}}$ and 
$T = 24$\;h and $N_{\text{bins}}$ 
the results are compatible with fluctuations 
around unity controlled by 
statistical uncertainties alone,
as indicated by the large KS probabilities.
The impact of systematic errors appears to be minimal, 
as the statistical uncertainties are comparable 
to the one-sigma spread. 
In such a setting, constraints on 
the SME coefficients could reasonably be
extracted using only statistical uncertainties.
However, these results are insufficient to
conclude that systematic uncertainties can 
be neglected when looking at sidereal and solar 
distributions with SME-sensitive $x_c$ 
ratios~\eqref{eq:rc},\eqref{eq:ra5}. 
This is because low- and high-$x$ 
regions, where the trigger behaves
quite differently and is affected 
by the instantaneous luminosity,
can expect a marked difference 
in systematic effects between the 
beginning and end of each fill. 

As long as each bin is considerably smaller 
than the duration of a typical fill
(e.g., for $T=1$\;h, each bin is between $\sim$ half
a second ($N_{\text{bins}}=100$) 
and 15 min ($N_{\text{bins}}=4$),
it is expected that all such effects will average out. 
On the other hand, for the solar or sidereal phase, 
the time bins range between $\sim$ 15 min and 6 h.
It is possible that large fluctuations in 
trigger efficiencies and other systematics during 
the high-luminosity phase of the 
fill might result in residual non-negligible 
effects in the solar and sidereal distributions.
For example, if any systematic effects 
$\sim \mathcal{O}(15\;\text{mins})$ are present,
then comparisons between 
$T=1$\;h with $N_{\text{bins}} = 4$ and 
$T=24$\;h with $N_{\text{bins}} = 100$ 
(thus probing similar blocks in time)
may be useful. 


\subsection{$x_c$ phase-space analysis}
\label{ssec:xc_analysis}
%
When splitting the phase space in cuts above and
below $x_c = 10^{-3}$ the normalized counts in the
three panels of Fig.~\ref{fig:DIS-0.001} strongly
resemble the $Q_c$ cuts in Fig.~\ref{fig:DIS-20}.
Similarly, in light of discussion in Sec.~\ref{ssec:initial}, 
it is expected that the $T=1$\;h distributions for the ratios 
$r(x> x_c , x< x_c )$ given explicitly 
in Eqs.~\eqref{eq:rc},\eqref{eq:ra5} 
will be distributed around unity and 
dominated by statistics.
As discussed, any potential solar and sidereal effects 
are washed out when 
binning data using a test period 
much smaller than 24 h.
This is indeed the case as can be seen 
by the results presented in 
Figs.~\ref{fig:KS-test-x-1-4} and \ref{fig:KS-test-x-5-8}. 
In contrast to the $Q_c$ distributions for all phases, 
the sidereal and solar phases for the $x_c$ distributions
contain more structure. This is immediately
evident in the solar phases, 
Figs.~\ref{fig:KS-solar-x-1-4} and \ref{fig:KS-solar-x-5-8}. 
Several bin configurations exhibit small KS
probabilities, suggesting the presence of unaccounted
for systematics. This is also visually apparent, 
as the one-sigma spread, particularly for small-medium
$N_{\text{bins}}$, is much wider than the error bars on the
central values with accompanying larger deviation around
unity than in the test-phase case. Some 
of these effects are inherited in the sidereal distributions,
as is also observed in 
Figs.~\ref{fig:KS-sidereal-x-1-4} and \ref{fig:KS-sidereal-x-5-8}. 
However, in contrast to the solar-phase case, 
much larger KS
probabilities are consistently observed.
This is still not enough to conclude
missing systematic effects are 
genuinely solar in origin.
The estimate of the systematic contribution 
for a given $N_{\text{bins}}$ is obtained
by calculating $\sqrt{\sigma^2 - \sigma^2_{\text{stat.}}}$, 
where $\sigma$ is the $1-\sigma$ spread 
and $\sigma_{\text{stat.}}$ is the mean statistical error
of the distribution central values. 

It is important to stress that the 
observed systematic effects 
are not directly connected to 
the large fluctuations of the instantaneous
luminosity nor have been 
previously observed 
(systematic errors at the sub-percent
level have had a negligible 
impact on previous ZEUS analyses). 
A direct confirmation
of this result can be obtained 
by means of a Monte Carlo study. 
In particular, inclusive DIS events 
with $Q^2 > 4 \;\text{GeV}^2$ have been 
generated using the Monte Carlo
ARIADNE~\cite{Pettersson:1988zu, 
Lonnblad:1988nh, Lonnblad:1989kj}. 
The events have been subsequently
passed through the ZEUS detector 
and trigger simulations 
based on GEANT 3~\cite{Brun:1987ma}.

The parton-level calculation is purely 
Standard Model and does not 
introduce any direct time
dependence: the generated events 
do not possess time stamps. At the same 
time, the detector response and the 
trigger configuration depend on the 
instantaneous luminosity and change
over time. Data events are grouped into 
blocks with definite detector and 
trigger configurations
and, for each of these blocks, Monte Carlo 
events have been appropriately generated.
In order to include time dependence 
in the Monte Carlo events and to 
perfectly simulate the impact
of the variable instantaneous luminosity 
over the course of five years the 
following procedure
is followed. For each luminosity block, 
containing a given number of data events, 
all time stamps are extracted and 
assigned to random Monte Carlo events 
(selected from all those events generated
with the correct detector and trigger status). 
The obtained Monte Carlo sample 
simulates perfectly any
time dependence associated with the 
instantaneous luminosity and to 
the conditions of the detector, to the
extent of which the detector 
simulation accurately reproduces the 
response of the actual detector.

This study has been performed on 
a subset of all data (namely electron 
data taken in 2006) corresponding
to an integrated luminosity of 
54.8 pb${}^{-1}$. Comparisons between 
data and Monte Carlo for this sample are shown
for the test phase in Figs.~\ref{fig:MC-test-x-1-4},
\ref{fig:MC-test-x-5-8}, 
solar phase in Figs.~\ref{fig:MC-solar-x-1-4},
\ref{fig:MC-solar-x-5-8}, and sidereal phase
in Figs.~\ref{fig:MC-sidereal-x-1-4},
\ref{fig:MC-sidereal-x-5-8}.
A crucial observation is that phase 
distributions obtained from Monte Carlo 
events are perfectly compatible with
statistical uncertainties alone: 
no evidence of any residual 
systematic contribution to the
fluctuation of the binned central 
values around unity is 
observed in these simulations.
This result is also immediately visible 
by comparing the one-sigma spreads of 
data and Monte Carlo, with the former
being much larger than the 
latter (and the latter being in 
agreement with the statistical errors alone).

This analysis suggests that the residual 
systematic errors observed in data 
are not modeled in existing Monte Carlo
simulations. As explained above, 
a reasonable strategy is to simply 
use the difference in quadrature 
between the one-sigma spreads and the 
corresponding statistical errors as 
an estimate of these additional systematics.
Note that, in the present study, 
all previously known sources of systematic 
uncertainties cancel, as demonstrated
by the lack of such 
effects in the Monte Carlo study.

As an additional check, separate studies involving 
events taken under HIGH or LOW 
trigger settings, which are constant
within each luminosity block, 
have been performed and no 
discernible impact on the presence 
of the systematic uncertainties
discussed above can be observed. In particular, 
the vast majority of events have 
been recorded under HIGH trigger conditions 
which consequently
dominate all the presented distributions.


\subsection{Constraints and discussion}

\label{ssec:constraints}
%
The analysis in Sec.~\ref{ssec:xc_analysis}
clearly indicates the presence of an unknown, 
substantial, and pervasive time-dependent 
systematic effect.
Consistently low KS probabilities 
and large systematic errors relative 
to $T_{\text{sid.}}$ and
$2T_{\text{solar}}-T_{\text{sid.}}$ are observed
and suggestive of a possible unaccounted 
for solar-periodic effect
clearly not attributable to Lorentz violation. 
While no claim can be made at this stage of a genuine 
solar signature, there is no significant 
indication of a comparable sidereal effect.
Taken together, the extracted sidereal systematics 
may therefore reflect the dilution of the observed
potential solar-periodic effect. This establishes
a baseline for extracting constraints: a conservative 
approach to estimating the upper limit on 
the total sidereal error is to combine 
in quadrature the statistical errors 
with the (larger) solar systematics. 
For all distributions, 
the case $N_{\text{bins}} = 4$ yields 
the smallest statistical errors and 
thus the largest representative effect
of underlying systematics. Thus, for the
solar distributions, the systematics
extracted ($\sim 0.24\%$) are taken as a representative
value to add to the sidereal statistics in quadrature.
A fuller understanding of this (until now, unknown) 
systematic effect is left for 
future detailed studies 
beyond the scope of the present analysis.

To extract constraints, the following procedure is performed. 
The ratios~\eqref{eq:rc},\eqref{eq:ra5} must first have the
laboratory coefficients replaced with the
SCF coefficients as explained in Sec.~\ref{sec:sidsignals}.
The ratios then depend on the local sidereal angle 
$\theta_\oplus = \omega_\oplus T_\oplus$. For a given
bin $i$ the theoretical, ratios $r_i^{\text{thr.}}$ 
are are calculated for $N_{\text{bins}}$:
\begin{equation}
\label{eq:ri_theory}
r^{\text{thr.}}_i
= \frac{N_{\text{bins}}}{2\pi}
\int_{\frac{2\pi(i-1)}{N_{\text{bins}}}}
^{\frac{2\pi i}{N_{\text{bins}}}} 
r(x>x_c, x<x_c;\theta_\oplus)d\theta_\oplus,
\end{equation}
where $i=1,\cdots, N_{\text{bins}}$. 
This quantity can be compared directly 
the with experimental sidereal
ratios $r^{\text{exp.}}_i$ discussed in detail.
A $\chi^2$ function is constructed
\begin{equation}
\label{eq:chi2}
\chi^2 =
\frac{1}{\sigma_{\text{tot.}}^2}\sum_{i=1}^{N_{\text{bins}}}
\left(r^{\text{exp.}}_i 
- r^{\text{thr.}}_i\right)^2,
\end{equation}
for each of the 36 observable SCF coefficients and
95\% confidence-level (C.L.) constraints
are extracted one coefficient at time, 
in line with standard procedure~\cite{tables}.

The results are presented in Tables~\ref{tab:cbounds}
and~\ref{tab:a5bounds}.
Comparing to existing limits tabulated 
in Ref.~\cite{tables} is informative.
For the $c_f^{\mu\nu}$ coefficients with flavor $f=u,d$, 
the results derived here represent the first 
constraints on coefficient combinations
sensitive to sidereal oscillations, or combinations that
violate rotation invariance. 
The existing and in some cases considerably 
more stringent limits in Table D37 of Ref.~\cite{tables} 
apply to a special case 
of rotation-invariant coefficient combinations 
using cosmic-ray observations~\cite{Schreck:2017isa}. 
Such constraints also rest on a number
of model-dependent assumptions, so direct comparison between
those results and what is 
presented here should be made with caution.
Electrons and protons can in principle have $c$-type coefficients as
well. Clock-comparison and related 
experiments have constrained
these species of coefficients at 
levels below $10^{-20}$. 
For the $a^{(5)}$-type coefficients 
the results here are complete
first limits. One potential point 
of comparision would be the 
effective $a^{(5)}$-type coefficients for 
protons, described
in Table D11 of Ref.~\cite{tables}. 
Using hydrogen 1S-2S transitions,
constraints on similar combinations 
of proton coefficients
are currently at the 
level of $10^{-7}$-$10^{-8}$\;GeV$^{-1}$, which is
similar in magnitude to what is found for the $u$-quark 
$a^{(5)}$-type coefficients~\cite{Kostelecky:2015nma}.


==> ZEUS_LV-aut.tex <==
%=================================================================== 
%
%  This file will be replaced with the "official" author
%  list which is created for each ZEUS paper individually.
%
%===================================================================== 
\pagenumbering{Roman} 

\begin{center} 
{\Large  The ZOOPS Collaboration}
\end{center}

{\raggedright
  F.~Author$^{1}$,
  A.~Nother,
  X.~Whoever\\
 {\it Absolutely Non-Existing Institute of Nothing, Nowhere, Country}~$^{a}$ 
}

\par\filbreak
\begin{supertabular}[h]{rp{14cm}}
$^{\ 1}$ & now visiting a scientist next door\\ 
\end{supertabular}

\begin{tabular}[h]{rp{14cm}}
$^{a}$ &  supported by the National Council of Nonsense (NCNS)\\ 
\end{tabular} 


==> ZEUS_LV-cit_nomcite.tex <==
%==============================================================================
% Some definitions of citations
%==============================================================================
%------------------------------------------------------------------------------
% -> CTD
%------------------------------------------------------------------------------
\def\citeCTD{{\cite{%
nim:a279:290,npps:b32:181,nim:a338:254%
}}\xspace}
%------------------------------------------------------------------------------
% -> MVD
%------------------------------------------------------------------------------
\def\citeMVD{{\cite{%
nim:a581:656%
}}\xspace}
%------------------------------------------------------------------------------
% -> STT
%------------------------------------------------------------------------------
\def\citeSTT{{\cite{%
nim:a535:191%
}}\xspace}
%------------------------------------------------------------------------------
% -> CAL
%------------------------------------------------------------------------------
\def\citeCAL{{\cite{%
nim:a309:77,nim:a309:101,nim:a321:356,nim:a336:23%
}}\xspace}
%------------------------------------------------------------------------------
% -> HES
%------------------------------------------------------------------------------
\def\citeHES{{\cite{%
nim:a277:176%
}}\xspace}
%------------------------------------------------------------------------------
% -> 6mT
%------------------------------------------------------------------------------
\def\citeSixmT{{\cite{%
thesis:gosau:2007%
}}\xspace}
%------------------------------------------------------------------------------
% -> BAC
%------------------------------------------------------------------------------
\def\citeBAC{{\cite{%
nim:a300:480%
}}\xspace}
%------------------------------------------------------------------------------
% -> LUMI
%------------------------------------------------------------------------------
\def\citePCAL{{\cite{%
desy-92-066,zfp:c63:391,acpp:b32:2025%
}}\xspace}
\def\citeSPECTRO{{\cite{%
nim:a565:572%
}}\xspace}

